Classification and Feasibility Assessment of Infinitely Many Iso-Impulse Three-Dimensional Trajectories

In two-body dynamics, it is proven that for a sufficiently long flight time, generating infinitely many iso-impulse solutions is possible by solving a number of $\Delta v$-allocation problems analytically. A distinct feature of these solutions is the existence of two impulse anchor positions (APs) that correspond to the locations of the impulses on time-free, phase-free, base solutions. In this paper, the existence and utility of three-impulse base solutions are investigated and their complete solution spaces are characterized and analyzed. Since two- and three-impulse base solutions exist, a question arises: How many APs should base solutions have? A strategy is developed for choosing base solutions, which offers a certificate for $\Delta v$ optimality of general three-dimensional time-fixed rendezvous solutions. Simultaneous allocation of $\Delta v$ at two and three APs is formulated, which allows for generating $\Delta v$-optimal solutions while satisfying a constraint on individual impulses such that $\Delta v \leq \Delta v_\text{max}$. All iso-impulse solutions are classified in four layers: 1) base solutions, 2) feasible solution spaces, 3) solution families, and 4) solution envelopes. The method enables us to characterize the complete solution space of minimum-$\Delta v$, iso-impulse, three-dimensional trajectories under the nonlinear two-body dynamics. To illustrate the utility of the method, interplanetary and geocentric problems are considered.

==> SolutionEnvelopeEquations.tex <==
\subsection{Generation of Solution Envelopes}\label{sec:sol_env}
%The concept of solution envelope is informative. 
%It determines the solution space for a solution family (that correspond to a fixed number of orbital revolutions on the four phases of the maneuver). 
Solution envelopes introduced by Saloglu et al. 
 \cite{saloglu_existence_2023} represent the complete space of orbital period values of the phasing orbits of all infinity of iso-impulse solutions. 
 %More specifically, it is possible to determine the range of the orbital periods of the phasing orbits as a function of the orbital period of the initial orbit. 
 We have shown that solution envelopes take polygonal shapes, which means that the vertices of the solution envelopes contain sufficient data for characterizing and visualizing them. Analytic relations for determining the corner points of these solution envelopes have to be modified depending on the number of impulse APs, which extends the work in \cite{saloglu_existence_2023}. This modification is required since the $TOP_p$ can be distributed between two or three impulse APs simultaneously. The procedure for introducing phasing orbits at two or three distinct impulse APs is not coupled through the $\Delta v_\text{total}$ requirement. This decoupling requires a special treatment compared to the case when phasing orbits are added at the same impulse AP. To precisely determine the solution envelopes, we have to answer two questions. First, when $T_{1,1}$ takes its minimum value, i.e., $T_0$, we have to answer the following questions: 
\begin{enumerate}
\item What are the maximum and minimum values of orbital periods for the remaining phasing orbits?
\item What are the values of orbital periods, when $T_{1,1}$ takes its maximum value? 
\end{enumerate}

With these questions in mind, three corners have to be determined for each phasing orbit solution envelope. However, if any of these values are at the maximum or minimum boundary that can be taken at the corresponding impulse AP, there is a possibility for one additional corner point. When we consider the second and third APs, the relations to determine corner points are similar. When generating solutions, different AP phasing orbits are not related in terms of total $\Delta v$. 
Therefore, for the first AP, we treat the second, and third AP phasing orbit periods as constant parameters and subtract them from the available time for phasing orbits, $TOF_p$. 

Given the above explanation, we start by determining the leftmost corners, where $T_{1,1} = T_0$ for the first AP. The minimum values of orbital periods at the first AP are
\begin{equation}
    \begin{aligned}
        T_{n_{p,1},1,\text{min}} &= \frac{TOF_p - N_{1,1}T_{1,1,\text{min}} - C_1}{\sum_{k=2}^{n_{p,1}}N_{k,1}}, & & 
        T_{s,1,\text{min}} = \frac{TOF_p - N_{1,1}T_{1,1,\text{min}} - \sum_{k=s+1}^{n_{p,1}}N_{k,1}T_{k,1,\text{max}} - C_1}{\sum_{k=2}^{s}N_{k,1}},
    \end{aligned}
    \label{eq:env_min_ap1}
\end{equation}
where $s=2,\cdots,n_{p,1}-1$, and $C_1 = \sum_{k=1}^{n_{p,2}}N_{k,2}T_{k,2,\text{max}} + \sum_{k=1}^{n_{p,3}}N_{k,3}T_{k,3,\text{max}}$. If any of the $T_{s,1,\text{min}}$ values is less than $T_0$, then we set them to $T_0$. Then, we obtain the maximum orbital period values at the first AP by
\begin{equation}
    \begin{aligned}
        T_{m,1,\text{max}} = \frac{TOF_p - \sum_{k=1}^{m-1}N_{k,1}T_{k,1,\text{min}} - C_2}{\sum_{k=m}^{n_{p,1}}N_{k,1}},
    \end{aligned}
    \label{eq:env_max_ap1}
\end{equation}
where $m=2,\cdots,n_{p,1}$ and $C_2 = \sum_{k=1}^{n_{p,2}}N_{k,2}T_{k,2,\text{min}} + \sum_{k=1}^{n_{p,3}}N_{k,3}T_{k,3,\text{min}}$. If any of these maximum values are larger than the upper bound, $T_{k,1}(\alpha_{k,1} = 1)$, we set them equal to the upper bound. The maximum value of $T_{1,1}$ is when all the orbital periods of phasing orbits at the first AP are equal, which can be written as, 
\begin{equation}
    T_{1, 1, \text{max}}=\frac{TOF_p-C_2}{\sum_{k=1}^{n_{p,1}} N_{k,1}}.
    \label{eq:env_maxT1_ap1}
\end{equation}

Proceeding to the second AP, maximum and minimum values can be determined when $T_{1,1} = T_0$ as,
\begin{equation}
    \begin{aligned}
        T_{m,i,\text{max}} &= \frac{TOF_p - \sum_{k=1}^{m-1}N_{k,i}T_{k,i,\text{min}} - C_{3,q}}{\sum_{k=m}^{n_{p,i}}N_{k,i}}, \\
        T_{n_{p,i},i,\text{min}} &= \frac{TOF_p-N_{1,1}T_{1,1,\text{min}}- C_{4,q}}{\sum_{k=1}^{n_{p,i}}N_{k,i}},\\
        T_{s,i,\text{min}} &= \frac{TOF_p -N_{1,1}T_{1,1,\text{min}}- \sum_{k=s+1}^{n_{p,2}}N_{n_{p,i},i}T_{n_{p,i},i,\text{max}} - C_{4,q}}{\sum_{k=1}^{s}N_{k,i}},   
    \end{aligned} \quad \text{for} \quad i = 2,3,
    \label{eq:solspace_2AP_3AP_eq}
\end{equation}
where $m = 2,\cdots,n_{p,i}$, and $s=1,\cdots,n_{p,i}-1$ and 
\begin{align*}
    C_{3,q} & = \sum_{k=1}^{n_{p,1}}~N_{k,1}~T_{k,1,\text{min}} + \sum_{k=1}^{n_{p,q}}~N_{k,q}~T_{k,q,\text{min}}, \\
    C_{4,q} & = \sum_{k=2}^{n_{p,1}}~N_{k,1}~T_{k,1,\text{max}} + \sum_{k=1}^{n_{p,q}}~N_{k,q}~T_{k,q,\text{max}},
\end{align*}
with $q = 3$ if $i = 2$ or vice versa. Note that the minimum and maximum values we use in $C$ constants are the upper and lower bounds those orbital periods possibly can take.
To calculate the maximum value of the first orbit, when $i \in \{2,3\}$, we have
\begin{equation}
    T_{1, i, \text{max}}=\frac{TOF_p-C_{3,q}}{\sum_{k=1}^{n_{p,i}} N_{k,i}}.
    \label{eq:env_maxT1_ap23}
\end{equation}

If any of the resultant values are not between the bounds, then the upper or lower bound is set for the corresponding orbital period value. In the case of the upper bound, there is a possibility of having one additional corner in the solution envelope. That corner is at the point when $T_{1,1}$ is maximized when the other orbital period is at its maximum bound. The other case is when the minimum value of the orbital periods is higher than its lower bound when $T_{1,1} = T_0$. Therefore, there exists a corner where the orbital period value decreases and takes its minimum value at a point when $T_{1,i} \neq T_0$.
When there is a possibility of having a corner point due to an orbital period variable being on the upper bound, one can determine this point by maximizing $T_{1,1}$ when $T_{j,1}$ is at the maximum value for any $j = 2,\cdots,n_{p,1}$, 
\begin{equation}
\begin{aligned}
    T_{1,1,\text{max}} &= \frac{TOF_p - N_{j,1}~T_{j,1,\text{max}}-C_2}{\sum_{k=1}^{j-1}N_{k,1}}, \quad \text{for}\quad j = n_{p,1}, \\
    T_{1,1,\text{max}} &= \frac{TOF_p -\sum_{k=j}^{n_{p,1}}N_{k,1}~T_{k,1,\text{max}} -C_2}{\sum_{k=1}^{j-1}N_{k,1}}, \quad \text{for}\quad j \neq n_{p,1}.
    \end{aligned}
    \label{eq:env_corner1_ap1}
\end{equation}

If an additional corner is possible due to $T_{j,1,\text{min}}$ being greater than the lower bound, we have 
\begin{equation}
\begin{aligned}
     T_{1,1} = T_{j,1,\text{min}} &= \frac{TOF_p -C_1}{\sum_{k=1}^{j}N_{k,1}}, \quad \text{for}\quad j = n_{p,1}, \\
     T_{1,1} = T_{j,1,\text{min}} &= \frac{TOF_p -\sum_{k=j+1}^{n_{p,1}}N_{k,1}~T_{k,1,\text{max}} -C_1}{\sum_{k=1}^{j}N_{k,1}}, \quad \text{for}\quad j \neq n_{p,1}.
    \end{aligned}
    \label{eq:env_corner2_ap1}
\end{equation}

At the second or third AP, similar relations can be derived for corner points for the case when any of the variables are at the upper bound: 

\begin{equation}
\begin{aligned}
    T_{1,1,\text{max}} &= \frac{TOF_p - N_{j,2}~T_{j,2,\text{max}}-\sum_{k=1}^{j-1}N_{k,2}~T_{k,2,\text{min}} - \sum_{k=1}^{n_{p,3}}N_{k,3}~T_{k,3,\text{min}}}{\sum_{k=1}^{n_{p,1}}N_{k,1}}, \quad \text{for} \quad j = n_{p,2}, \\
    T_{1,1,\text{max}} &= \frac{TOF_p -\sum_{k=j}^{n_{p,2}}N_{k,2}~T_{k,2,\text{max}} - \sum_{k=1}^{j-1}N_{k,2}T_{k,2,\text{min}}-\sum_{k=1}^{n_{p,3}}N_{k,3}~T_{k,3,\text{min}}}{\sum_{k=1}^{n_{p,1}}N_{k,1}}, \quad \text{for} \quad j \neq n_{p,2},
    \end{aligned}
    \label{eq:env_corner1_ap2_ap3}
\end{equation}
where the subscripts $(., 2)$ and $(.,3)$ can be swapped to determine the corner points for the third AP. 

There can be a corner point due to the $T_{j,2,\text{min}}$ or $T_{j,3,\text{min}}$ taking values greater than the lower bound for any $j$. If such a case is possible, the additional corner is at the point of minimum value of $T_{1,1}$ when $T_{j,2,\text{min}}$ or $T_{j,3,\text{min}}$, which are the lowest values they can get, regardless of the value of $T_{1,1}$. Unlike the first AP case, $T_{1,1} \neq T_{j,2, \text{min}}$ or  $T_{1,1} \neq T_{j,3, \text{min}}$ because $T_{1,1}$ is not related to other AP phasing orbits through total $\Delta v$. At this corner point, the minimum value of $T_{1,1}$ is determined by 
 \begin{equation}
 \begin{aligned}
      T_{1,1} &= \frac{TOF_p - \sum_{k=1}^{j}N_{k,2}~T_{k,2,\text{min}} - \sum_{k=j+1}^{n_{p,2}}N_{k,2}~T_{k,2,\text{max}}-T_{n_{p,1},1,\text{max}} - \sum_{k=1}^{n_{p,3}}N_{k,3}~T_{k,3,\text{max}}}{\sum_{k=1}^{n_{p,1}-1}N_{k,1}}, \quad \text{for} \quad j \neq n_{p,i}, \\
       T_{1,1} &= \frac{TOF_p - \sum_{k=1}^{j}N_{k,2}~T_{k,2,\text{min}} -T_{n_{p,1},1,\text{max}} - \sum_{k=1}^{n_{p,3}}N_{k,3}~T_{k,3,\text{max}}}{\sum_{k=1}^{n_{p,1}-1}N_{k,1}}, \quad \text{for} \quad j = n_{p,i}.
     \end{aligned}
     \label{eq:env_corner2_ap2_ap3}
 \end{equation}

Alternatively, all these solution envelopes can be determined by solving a set of linear programming problems by changing the objective of the problem for each corner point. For instance, the minimum and maximum values of $T_{2,2}$ when $T_{1,1}=T_0$ are determined by minimizing and maximizing the corresponding element of the design variable vector. Design variables consist of all the phasing orbit orbital period parameters at all the APs, $\boldsymbol x = [T_{1,1}, \cdots, T_{n_{p,1},1}, T_{1,2}, \cdots, T_{n_{p,2},2}, T_{1,3}, \cdots, T_{n_{p,3},3}]$ where their upper and lower bounds are known. The linear equality constraint is the total $TOF$ constraint given in Eq.~\eqref{eq:TOF_gen} and linear inequality constraints are $T_{k,i} \leq T_{k+1,i}$ for each $k = 1,\cdots, n_{p,i}$ where $i \in \{1, 2, 3\}$. We have used a linear programming formulation to obtain the analytic relations and verify the obtained solution envelopes. 




% ABSTRACT VERSION EQUATIONS %%
%% THESE ARE OLD EQUATIONS AND SHOULD REMAIN COMMENTED %%
% Let $n_t = n_{p,1} + n_{p,2}$,

% \begin{equation}
% \begin{aligned}
% T_{s, \min } &=T_0, \quad 
% T_{n_t,\text{min}} =T_{\text{pf}} \quad
% T_{n_t, \text{max}} =T_f, \\
% T_{1, \text{max}}&=\frac{TOF_p-N_{n_t} T_{n_t}}{\sum_{k=1}^{n_t-1} N_k}, \\
% T_{m,\text{max}}&=\frac{TOF_p - \sum_{k=1}^{m-1} N_k T_{k,\min} -N_{n_t}T_{n_t,\min}}{\sum_{k=m}^{n_{t-2}} N_k}, \\
% \end{aligned}
% \end{equation}
% where $s = 1, \cdots, n_t-2$, and $m = 2, \cdots, n_t-2$. When the value of $T_{n_t}$ is at the maximum bound, there is a corner at the solution space. The orbital period values at the corner point are calculated as 

% \begin{equation}
% T_1=T_{n p-1}=\frac{TOF_p -N_{n_t} T_{n_t, \max }}{\sum_{k=1}^{n_{t}-2}N_k}.
% \end{equation}

% When there is a corner in the solution space, $T_{n_t-1,\max}$ and $T_{n_t-1,\max}$ is calculated using 

% \begin{equation}
% \begin{aligned}
% T_{n_{t, 2}, \max }&=\frac{TOF_p -\sum_{k=1}^{n_{t-2}} N_k T_{k, \min }-N_{n_t} T_{n_t, \min }}{N_{n_{t-2}}}, \\
% T_{n_{t-1}, \min }&=\frac{TOF_p-N_{n_t} T_{n_t, \max }-N_1 T_{1, \min }}{\sum_{k=2}^{\n_{p-1}} N_k} .\\
% \end{aligned}
% \end{equation}

==> intro_long.tex <==
\section{Introduction}
 %One of the goals of the space agencies is to create human establishments around the moon and perform crewed missions to Mars and beyond. 
 %The design of spacecraft optimal trajectories, with respect to various optimality criteria such as flight time and propellant consumption, is an essential step in space mission design for accomplishing mission goals \cite{strange2002graphical,ellison2018application}. 
 The optimization of spacecraft trajectory in terms of flight time and propellant consumption is an essential step in space mission design for accomplishing mission goals~\cite{strange2002graphical,ellison2018application}.
 In addition, many optimal trajectories are generated for estimating the mass budget and launch cost during the preliminary spacecraft design process \cite{woolley2019optimized,woolley2019cargo}. Spacecraft trajectories are significantly influenced by their propulsion systems, which can be classified broadly as chemical rockets \cite{olympio2009designing}, solar-powered electric propulsion systems \cite{taheri2016enhanced,petukhov2019joint,arya2021composite} and propellant-free systems (e.g., solar sails) \cite{shirazi2018spacecraft}. A variety of numerical methods exist for solving spacecraft trajectory optimization problems based on indirect and direct solution methods~\cite{bertrand2002new,ross2007low,taheri2012shape,taheri2016initial,taheri2015fast,zhu2017solving,englander2017automated,taheri2018shaping,taheri2018generic,pan2020practical,taheri2021costate,li2021homotopy,nurre_comparison_2022,oguri2022solar,ayyanathan2022mapped,mannocchi2022homotopic,zhang2023solution,nurre2023duty}. The indirect methods use the necessary conditions from calculus of variations whereas the direct method discretizes the continuous problem into a parametric optimization problem~\cite{betts_survey_1998,conway_survey_2012}. Indirect methods require solving two-point boundary value problems that require determining the initial costates to solve which can be sensitive even though the optimal control can be determined analytically. The direct methods do not require the knowledge of optimal control theory and it is easier to incorporate path and control constraints but require an initial guess for the solver to improve upon.  
 
 Impulsive trajectory optimization problems are an important class of spacecraft trajectory optimization especially for crewed missions, as they require shorter mission times compared to low-thrust trajectories~\cite{shirazi_spacecraft_2018}. Determining when and where to apply a finite, yet unknown number of impulses is the main task for generating extremal impulsive trajectories. Early work on impulsive trajectories often categorizes solutions concerning initial and target orbit shape and utilizes analytical methods~\cite{gobetz_survey_1969}. The Hohmann transfer produces the optimal solution for planar circular-to-circular transfers with two impulses tangential to the velocity at the apse points~\cite{hohmann_attainability_1960}. After a certain ratio of the initial and final orbits, the bi-elliptic transfer, which requires three impulses, produces less $\Delta v$ than the Hohmann transfer~\cite{edelbaum1959some}. The bi-parabolic transfer is the theoretical limit of three-impulse trajectories when the midcourse impulse is performed at infinity~\cite{vallado_fundamentals_2001}. It is shown that for transfer between coaxial planar ellipses, at most three impulses are required~\cite{ting1960optimum}. Some of the surveys on early work for impulsive trajectory optimization can be found in Ref.~\cite{edelbaum_how_1966, gobetz_survey_1969}. Recent investigations include the trajectories of the planar elliptic transfers. Pontani~\cite{pontani_simple_2009} investigated and proved the global optimality of two and three-impulse (with the maximum apoapsis radius) trajectories for transfers between coplanar, coaxial elliptical orbits and showed that the selection can be made depending on the apoapsis and periapsis radii of terminal orbits. Carter and Humi proposed the closed-form solutions of optimal two and three-impulse when the terminal ellipses are coaxial for the planar case~\cite{carter_two-impulse_2020}. They also use a transformation to have linear equations of motion to investigate the time-free and time-fixed transfer between planar ellipses with two and three-impulses~\cite{carter_generalized_2021}. The nonaxial planar elliptical transfers are solved by a simplified optimization algorithm based on primer vector theory which implements a homotopic approach starting from a two-impulse Hohmann solution~\cite{li_minimum-fuel_2024}. 
 %whereas, for the three-impulse, they show that the bielliptic is never optimal, but it can get arbitrarily close to the bi-parabolic transfer~\cite{carter_two-impulse_2020}. ~\cite{carter_generalized_2021,li_minimum-fuel_2024}. 
 % Pontani,2009 Carter and Humi 2020, 2021, % [23]-[29] of thesis; 2024 paper by Li
 
 One of the methods to determine the number of impulses, impulse locations, and directions is to use the primer vector theory~\cite{lawden_optimal_1963}, which constitutes a set of first-order necessary conditions for the local optimality of impulsive solutions. Using the primer vector theory, a Nonlinear Programming (NLP) problem is formulated to obtain optimal impulsive trajectories~\cite{jezewski_efficient_1968}. The continuity in the position is typically ensured by solving Lambert's problem~\cite{battin_lamberts_1977, gooding_procedure_1990}. Different methods exist that solve Lambert's problem for optimal impulsive trajectories. Many short-arc embedded Lambert problems can be solved within multiple segments which avoids determining the location of impulses~\cite{ottesen_unconstrained_2021}. The process of obtaining an extremal solution based on primer vector theory starts with solving two- or many-impulse problems with the formulated NLP problem. Once a solution is obtained, the primer vector time history is inspected to ensure that the necessary conditions are satisfied. If there are one or multiple violations of the necessary conditions, an impulse is inserted at that time instant and the problem is resolved~\cite{sandrik_primer-optimized_nodate, bell_primer_nodate, chiu_optimal_nodate}. Primer vector is also used for impulsive rendezvous between close, circular, coplanar orbits for time-fixed problems~\cite{ prussing_optimal_1986,prussing_optimal_2003}. Hughes et al. compared the direct and primer vector based indirect optimization and concluded that the methods are not superior to each other~\cite{hughes_comparison_2003}.

Broad-search (meta-heuristic) algorithms consider a large decision space where the number, location, and direction of impulses can be a design variable. This offers flexibility for solving different types of problems, which might include multiple flyby and gravity-assist maneuvers~\cite{izzo_search_2007,campagnola_fast_2010, landau2018efficient}. Automated-design methods oftentimes utilize the usage of evolutionary algorithms~\cite{englander_automated_2012}. Evolutionary algorithms usually do not require an initial guess and can be used to generate impulsive trajectories for different numbers of impulses to determine the global optimal solutions and their corresponding number of impulses~\cite{abdelkhalik_n-impulse_2007,pontani_particle_2012,shen_global_2015,rosa_sentinella_cooperative_2009}. These algorithms can locate the global minimum rather than converging a local minimum in the neighborhood of the initial guess and they require a smaller set of discrete variables compared to nonlinear programs~\cite{conway_survey_2012}.

Numerical continuation-based methods can be used to determine the location of the impulses and the duration of the terminal coast arcs, which can serve as an initial guess to an NLP problem solver. 
%Numerical continuation-based methods first formulate the impulsive trajectory design problem as a low-thrust trajectory optimization problem while performing continuation on the magnitude of the thrust produced by the propulsion system. 
Once an initial ``low-thrust solution'' is obtained, a numerical continuation is performed on the maximum thrust acceleration value (or the maximum thrust parameter) such that the low-thrust solution gets closer to an impulsive solution as the thrust arcs get shorter~\cite{taheri_how_2020, taheri_acceleration-based_nodate}. An NLP problem can be formulated to solve the impulsive trajectory optimization problem with the initial guess for the impulse locations and times providing the sensitivity information using the primer vector theory~\cite{saloglu_acceleration-based_2022, arya_generation_2023}. 

In this context, the connection between the low-thrust and impulsive solutions is established with the notion of optimal switching surfaces, introduced by Taheri and Junkins~\cite{taheri_how_2020} to answer the ``How Many Impulses?'' question posed by Edelbaum~\cite{edelbaum_how_1966}. More specifically, Taheri and Junkins reported that for the problem of transferring a spacecraft from the Earth to asteroid Dionysus (Earth-Dionysus), four extremal impulsive solutions require the exact same total $\Delta v$. Therefore, it is shown that Edelbaum's ``How Many Impulses?'' question does not have a unique answer. Even though Taheri and Junkins considered fixed-type, rendezvous-type classes of maneuvers, there are some key features in the solutions of the Earth-Dionysus problem, including the fact that all impulses are applied at two distinct locations and that there is a fundamental arc common between all equal-$\Delta v$ solutions.  

The common features of the equal-$\Delta v$, multiple-impulse solutions of the Earth-Dionysus problem are investigated and explained by Saloglu et al.~\cite{saloglu_existence_2023, saloglu_existence_conf_2023}. It is shown that minimum-$\Delta v$ impulsive trajectories can be divided, at most, into four phases. More specifically, a broad classification of possible impulsive solutions is presented based on the time spent on four different phases: 1) the initial orbit, 2) a to-be-determined number of phasing orbits, 3) the phase-free arc, and 4) the final orbit. Given a fixed total time of flight, all possible impulsive solutions can be classified. In addition, it is shown that for the class of maneuvers with more than three impulses, it is possible to have infinitely many equal-impulse solutions, where the difference between each solution is due to the time spent on each phase of flight. These infinitely many solutions are represented by orbital period solution envelopes. Also, a unique, analytical $\Delta v$-feasibility algorithm is proposed. 

For long-time-horizon missions, impulsive trajectory optimization problems can be solved starting from a two-impulse, time-free, phase-free base solution, where impulse anchor positions (APs) are the positions at which the impulses occur on the base solution~\cite{saloglu_existence_2023}. At these impulse APs, impulses can be divided into multiple smaller-magnitude impulses. This way, thruster requirements can be satisfied without losing the $\Delta v$ optimality, and in some cases, only at the cost of requiring a maneuver that occurs over a longer flight time. Similarly, the phasing of the spacecraft on the geostationary orbit can be accomplished without considering additional phasing maneuvers~\cite{barea_dual-based_2022}. These smaller magnitude impulses put the spacecraft into several phasing orbits. A similar application of dividing an impulse into intermediate impulses, subimpulses, is shown in Ref.~\cite{barea_dual-based_2022} where they propose a dual-based optimization for impulsive maneuvers and compute the multi-impulse transfer from a two-impulse solution. In Saloglu et al.~\cite{saloglu_existence_2023}, the problem of dividing the impulse at an impulse AP is formulated as a $\Delta v$ allocation problem, which is solved analytically. This method is a substantially faster alternative compared to the continuation-based methods \cite{arya_generation_2023}. 
%Due to the analytic nature of the $\Delta v$- allocation problem, we were able to obtain infinitely many equal-$\Delta v$ optimal solutions for the Earth-Dionysus problem by recovering the minimum $\Delta v$ for the fixed-time rendezvous problem. The method starts by solving the most relaxed version of the problem, free-time transfer, and introduces phasing orbit and coast arcs to match the phasing and the mission total fixed time. 
%We concluded that the solutions can be classified by the number of revolutions on the different segments of the trajectory, namely, the initial orbit, target orbit, a phase-free arc, and a to-be-determined number of phasing orbits. 
The results presented in our previous study \cite{saloglu_existence_2023} motivated us to propose a more generalized approach to the design of impulsive maneuvers by introducing three-impulse free-time transfer which is relevant in spacecraft trajectories and appears frequently in circular-to-circular or elliptic-to-elliptic transfers.

The main contributions of this paper are as follows. 1) We consider maneuver scenarios with three-impulse, time-free, phase-free base solutions for obtaining infinitely many minimum-$\Delta v$ solutions. Classification of the solutions is presented in terms of the number of phasing orbits at possible APs and polygonal solution spaces are presented similar to the ones that are introduced in \cite{saloglu_existence_2023}. Similar to the bi-elliptic transfer between coplanar circular and coaxial elliptical orbits, there exists less $\Delta v$ solutions compared to the two-impulse case. By considering two- and three-impulse base solutions, we can cover all minimum-$\Delta v$ solution possibilities in a general, unified manner. 2) We previously introduced the $\Delta v$-allocation problem for a single AP that requires the maximum amount of impulse among the potential impulse APs. We extend the capabilities of our method by considering two and three APs. This allows us to divide the impulses simultaneously at any potential AP. We extend the feasibility discussion to the case when multiple APs are considered and visualize feasible solution space depending on the total number of revolutions that can occur on the phasing orbits. With the ability to consider multiple APs, we can extend the solution space and enable the option of dividing the impulse magnitude at multiple impulse APs, such that we gain authority in reducing all impulse magnitudes and making them realizable by thrusters.  Accommodating a threshold on the maximum $\Delta v$ value is an important operational ability and the proposed tool offers such a feature. 
%One of the main motivations for dividing the impulse value into smaller magnitude impulses is to satisfy the single impulse requirements of the thruster so that the trajectory is operationally realizable. %Therefore, if there exists a case where the amount of impulse is not realizable at more than one impulse AP, our proposed method allows us to make the solution feasible to a threshold on the maximum $\Delta v$ value. 
However, for problems with more constraints on the maximum value of impulse, it is inevitable to extend the time of maneuver if $\Delta v$-optimality is to be preserved especially for time-fixed cases. 
  

The paper is organized as follows. In Section~\ref{sec:genmultimp}, the $\Delta v$-allocation method to solve impulsive problems with a single AP is reviewed. The generation of three-impulse base solutions is explained in Section~\ref{sec:threeimpbase} and details on the selection process of two or three-impulse base solutions are explained. Then, formulations to consider multiple impulse APs, time-feasibility equations, and equations to produce solution envelopes are given in Section~\ref{sec:multianchor}.  In Section~\ref{sec:results}, numerical examples are provided to show how these methods are applied for generating interplanetary and planet-centric minimum-$\Delta v$ impulsive trajectories. Discussions on the selection of the base solution by numerical examples are given in Section~\ref{sec:discussion_base}. Finally, conclusions are given in Section \ref{sec:conclusion}.

